Work Practices and Perceptions from Women Core Developers in OSS Communities

The effect of gender diversity in open source communities has gained increasing attention from practitioners and researchers. For instance, organizations such as the Python Software Foundation and the OpenStack Foundation started actions to increase gender diversity and promote women to top positions in the communities. Although the general underrepresentation of women (a.k.a. horizontal segregation) in open source communities has been explored in a number of research studies, little is known about the vertical segregation in open source communities -- which occurs when there are fewer women in high-level positions. To address this research gap, in this paper we present the results of a mixed-methods study on gender diversity and work practices of core developers contributing to open-source communities. In the first study, we used mining-software repositories procedures to identify the core developers of 711 open source projects, in order to understand how common are women core developers in open source communities and characterize their work practices. In the second study, we surveyed the women core developers we identified in the first study to collect their perceptions of gender diversity and gender bias they might have observed while contributing to open source systems. Our findings show that open source communities present both horizontal and vertical segregation (only 2.3% of the core developers are women). Nevertheless, differently from previous studies, most of the women core developers (65.7%) report never having experienced gender discrimination when contributing to an open source project. Finally, we did not note substantial differences between the work practices among women and men core developers. We reflect on these findings and present some ideas that might increase the participation of women in open source communities.

==> 9_survey.tex <==
\begin{table*}[htb!]
    \centering
    \caption{Survey Questions}
    \label{tab:suggestion}
    \begin{tabular}{|p{0.45cm}|p{16.5cm}|} 
    \hline
ID & Question   
\\ \hline
Q1 &  In what group age are you?  
\\ \hline
Q2 & What is your workplace? 
\\ \hline
Q3 & How long have you been contributing to OSS Communities?
\\ \hline
Q4 & What is your education level?
\\ \hline
Q5 & What programming languages do you dominate? 
\\ \hline
Q6 & What communication channel do you use to conduct your interactions with other team members in OSS Communities?
\\ \hline
Q7 & How often do you usually interact with other team members in OSS Communities?
\\ \hline
Q8 & Are you happy with your participation in OSS Communities?
\\ \hline
Q9 & Do you agree that your contributions are well received in OSS Communities?
\\ \hline
Q10 & Have you ever felt that one of your contributions was not well received due to your gender? 
\\ \hline
Q11 & How often do you feel that your contributions were not well received due to your gender?
\\ \hline
Q12 & Do you think it is important to have gender diversity in OSS Communities?
\\ \hline
Q13 & What is your suggestion to increase women's participation in the OSS Communities?
\\ \hline
Q14 & In your opinion, how to create a more inclusive environment for women in OSS Communities?
\\ \hline
Q15 & In your opinion, what are the reasons that motivate women to contribute to the OSS Communities? 
\\ \hline
Q16 & In your opinion, are the use of engaging techniques relevant to attracting more women to OSS Communities?
\\ \hline
Q17 & Do you know about the current research on gender diversity in OSS Communities?
\\ \hline
Q18 & How do you perceive the relevance of gender diversity research in OSS Communities? 
\\ \hline
Q19 & After reading the title and abstract of the following research papers, how important do you evaluate their contributions?
\\ \hline
    \end{tabular}
    \end{table*}


